Sparsifying Distributed Algorithms with Ramifications in Massively Parallel Computation and Centralized Local Computation

We introduce a method for sparsifying distributed algorithms and exhibit how it leads to improvements that go past known barriers in two algorithmic settings of large-scale graph processing: Massively Parallel Computation (MPC), and Local Computation Algorithms (LCA). - MPC with Strongly Sublinear Memory: Recently, there has been growing interest in obtaining MPC algorithms that are faster than their classic $O(\log n)$-round parallel counterparts for problems such as MIS, Maximal Matching, 2-Approximation of Minimum Vertex Cover, and $(1+\epsilon)$-Approximation of Maximum Matching. Currently, all such MPC algorithms require $\tilde{\Omega}(n)$ memory per machine. Czumaj et al. [STOC'18] were the first to handle $\tilde{\Omega}(n)$ memory, running in $O((\log\log n)^2)$ rounds. We obtain $\tilde{O}(\sqrt{\log \Delta})$-round MPC algorithms for all these four problems that work even when each machine has memory $n^{\alpha}$ for any constant $\alpha\in (0, 1)$. Here, $\Delta$ denotes the maximum degree. These are the first sublogarithmic-time algorithms for these problems that break the linear memory barrier. - LCAs with Query Complexity Below the Parnas-Ron Paradigm: Currently, the best known LCA for MIS has query complexity $\Delta^{O(\log \Delta)} poly(\log n)$, by Ghaffari [SODA'16]. As pointed out by Rubinfeld, obtaining a query complexity of $poly(\Delta\log n)$ remains a central open question. Ghaffari's bound almost reaches a $\Delta^{\Omega\left(\frac{\log \Delta}{\log\log \Delta}\right)}$ barrier common to all known MIS LCAs, which simulate distributed algorithms by learning the local topology, \`{a} la Parnas-Ron [TCS'07]. This barrier follows from the $\Omega(\frac{\log \Delta}{\log\log \Delta})$ distributed lower bound of Kuhn, et al. [JACM'16]. We break this barrier and obtain an MIS LCA with query complexity $\Delta^{O(\log\log \Delta)} poly(\log n)$.

==> lcaMIS.tex <==
\section{Simulation in the LCA Model}
\label{sec:simu}
To obtain an efficient algorithm in the LCA model, our plan is to simulate the \algo{} algorithm from Section~\ref{sec:finegrained}.
One fundamental observation is, that whenever a node is super-heavy in some phase, we can perfectly predict its behavior.
In a sense, when we learn that some node is super-heavy in some phase, we do not need to waste queries to learn what its neighbors are doing in that phase.
The second crucial observation is, to be formalized soon, that a node that is \emph{not} super-heavy, has a relatively small amount of neighbors that beep at all in the corresponding phase.

We begin with a few words about the randomness that we use.
Notice that according to the design of our algorithm and due to the fact that we are executing $\bigO(\log \Delta)$ rounds, we will never need higher precision of randomness than $\bigO(\log \Delta)$ bits.
Thus, we assume that our random bit string is divided into $\bigO(\log^2 \Delta)$ pieces that yield every node independent $\bigO(\log \Delta)$ random bits per round (of the LOCAL algorithm) and furthermore, this information is available to the LCA at all times.
We think of the randomness $r_t(v)$ of node $v$ in round $t$ as a uniformly chosen number from the interval $[0, 1]$.
Hence, node $v$ beeps if $r_t(v) \leq p_t(v)$.

A second word about the model is about the type of query access we have to our input graph $G = (V, E)$.
In the introduction, we talked about the weakest kind of LCAs, where the queries return the $i$th neighbor of a node.
Our approach essentially always needs to query all neighbors of a given node and thus, from now on, we assume that the graph access is through an oracle that returns the whole adjacency list of a queried node.
Notice that this modification simply adds a $\Delta$ factor to the resulting query complexity as compared to the weaker model.


\paragraph{Set $S$ of Relevant Nodes in Phase $[t, t']$.}
Let us denote a phase that starts in round $t$ and ends in round $t' > t$ by $[t, t']$.
To simulate phase $[t, t']$ of length $t' - t = 2^i \cdot k$ for node $v$, the nodes that require us to take some action are the nodes that belong to the connected component induced by nodes that are not super-heavy and beep in phase $[t, t']$.
The set is defined through the following iterative process.
Start with set $S = \{v\}$.
Now, iterative, add any node $u$ adjacent to a node in $S$ if 
\begin{enumerate}
% 	\item $u$ is within distance $t' - t$ from $v$,
	\item not super-heavy, and
	\vspace{+3pt}
	\item $r_t(u) \leq p_t(u) \cdot 2^{2^i \cdot 5k} \cdot 2^{2^i \cdot k} = 2^{2^i \cdot 6k}$.
\end{enumerate}
Notice that if $u$ satisfies the second property, it will for sure not beep in phase $[t, t']$.
From that it follows that $S$ contains all the nodes that may join the MIS during the corresponding phase.

\subsection{A Warm-Up}
Next, we give an overview of how our simulation works on a high level and afterward, dive a bit deeper into formalities.
%The description is intentionally imprecise at times, in hopes of maximizing readability.

\paragraph{Example Simulation of Phase $[t, t']$.}
Let us make an oversimplifying assumption that we obtain $p_t(u)$ and $d_t(u)$ value whenever we perform a neighborhood query of $u$.
Let us even believe for now that simulating the set $S$ of nodes is enough for simulating phase $[t, t']$ of node $v$.
Given these simplifications, the LCA can find the set $S$ by querying nodes iteratively as given in the definition of $S$.
Notice that after simulating phase $[t, t']$, we need to return $p_{t'}(v)$ and whether $v$ is in the MIS or not.
Once our LCA knows the set $S$ and the $p_t$ values for all nodes, the simulation can be performed.
It can be the case that the set $S$ is large and there might be nodes further than $(t' - t)$-hops away from $v$ which cannot affect the simulation, but let us worry about that later.

\paragraph{Oracle Access.}
While the above toy-scenario might feel like it is far from serving our purpose, we can implement an algorithm that is almost as simple.
Our goal is to generalize the oracle answering adjacency list queries into two oracles that answer the questions: 
\begin{enumerate}
	\item ``What is the value $p_{t}(u)$ of node $u$ in the beginning of phase $[t, t']$?''
	\vspace{+3pt}
	\item ``What are the neighbors of node $u$ in the graph $G[S]$?''
\end{enumerate}
Let us denote an oracle that answers the first question by $\orc^{t}(u)$ and the second question by $\orc^{S}(u)$ and assume that we have a free access to both of them.
Then, the simulation of phase $[t, t']$ for node $v$ becomes again, quite simple.
The additional steps required (as compared to above) are to query each node $u$ with $\orc^{S}$ and $\orc^t$ to know whether it should be simulated or not and to obtain $p_t(u)$.
The price of the simulation, however, depends now on the query complexities of $\orc^t$ and $\orc^S$.
If $Q\left( \orc \right)$ is an upper bound on the complexity of any query to $\orc$, the resulting query complexity is $Q\left( \orc^S \right) \cdot Q\left(\orc^t \right) \cdot |S|$.

% We will show that this allows us to drop the query complexity of $\Delta^{\bigO(\log \Delta)} \cdot \log n$ given by the naive simulation down to $\Delta^{\bigO(\log \log \Delta)} \cdot \log n$.

\paragraph{Division to Subphases and Recursive Oracle Access.}
We are almost done with the informal description of our method.
The remaining step is to divide the phases into smaller subphases, until reaching a phase length of $k$.
To this end, the simulation of $[t_1, t_2]$ is divided into two parts.
Let us assume that phase $[t_1, t_2]$ is of length $2^i \cdot k = 2\ell$ for some $i > 0$ and let $t = t_1 + \ell$.
Denote the relevant nodes of the subphase $[t_1, t - 1]$ by $S_1$ and similarly for $[t, t_2]$.

Let us once again assume that we can access the oracles $\orc^{S_1}$ and $\orc^{t_1}$.
Similarly to the previous paragraph, we are able to simulate the subphase $[t_1, t - 1]$ in a straight-forward manner.
However, the subphase $[t, t_2]$ requires some care.
To provide subphase $[t, t_2]$ with query access to oracles $\orc^{S_2}$ and $\orc^{t}$, we \emph{encapsulate} $\orc^{S_1}$ and $\orc^{t}$ into new oracles as follows.
Whenever $\orc^{t}$ or $\orc^{S_2}$ is queried for node $u$, what happens behind the scenes is that the subphase $[t_1, t - 1]$ is simulated for $u$ using the oracle access to $\orc^{t_1}$ and $\orc^{S_1}$.
From the perspective of the simulation of subphase $[t, t_2]$, this is equivalent to having the oracle access to oracles $\orc^{t}$ and $\orc^{S^2}$.
Once again, this comes with a price.
The query complexity of simulating $[t, t_2]$ becomes $|S_2| \cdot \left( |S_1| \cdot Q(\orc^{t}) \cdot  Q(\orc^{S_1}) \right)$, where $|S_1|$ and $|S_2|$ stand, respectively, for upper bounds on the sizes of $S_1$ and $S_2$.

\paragraph{Some Notation.}
For phase $[t, t'] = q$ and node $v$, we denote $S_q(v) = S \cap N^{t' - t}(v)$, where $N^{\ell}(v)$ stands for the $\ell$-hop neighborhood of node $v$ in the input graph $G = (V, E)$.
We denote the graph $G\left[S_{q}\right]$ induced by nodes in the set $S_{q}$ by $\Gtt{t}{t'}$ and the maximum degree of $\Gtt{t}{t'}$ by $\Dtt{t}{t'}$.
Furthermore, let $N(S_q)$ be the set of nodes in $S_q$ and the neighbors of $S_q$ in the original graph $G$.

\subsection{The Roadmap for Simulation}
The goal of the rest of this section is to show the following things. 
% Next, we state two lemma, that show two things
First, we show that knowing set $S = S_{[t, t']}(v)$ is almost enough to fully simulate the behavior of node $v$ in phase $[t, t']$.
Then, we show that the deeper we go in the recursion and the shorter the (sub-)phases are, the smaller the maximum degree of $G[S]$ becomes.
The last step of the analysis of the simulation is to formalize the encapsulation of the oracles and then, we bound the number of queries in the whole process in Theorem~\ref{thm:numqueries}.
Finally, we observe that the nodes in the small components resulting from the shattering (Lemma~\ref{lemma:shattering}) are easy to handle.

% \paragraph{Simulating Super-Heavies}
% In the next lemma, we show that knowing the behavior of the set $S$ and the nodes neighboring it is enough to simulate phase $[t, t']$.
% An important observation is, that the nodes not in $S$ are either super-heavy or do not beep.
% Therefore, we know their behavior without having to know anything about their neighbors.
% Keeping this in mind, we imagine that we label

\begin{lemma}
	Consider the phase $q = [t, t']$, where $t' - t = \ell > 0$. 
	Let $S = S_q(v)$ and $S^* = N(S)$.
	Assume that our LCA is given $G[S^*]$ and the value $p_t(u)$ for every $u \in S^*$.
	Then, node $v$ can simulate its behavior in phase $q$.
	In particular, node $v$ learns $p_{t' + 1}(v)$ and whether it joined the MIS.
% 	\label{lemma:correctness}
\end{lemma}
\begin{proof}
	In essence, we have to argue that the behavior of nodes within the $\ell$-neighborhood of node $v$ that are not in $S^*$ cannot affect the outcome of phase $q$ for $v$.
	We argue by induction on the round index that the behavior of $v$ can be derived solely based on the nodes in $S^*$.
	The base case of round $t$ is clear since we are given $p_t(v)$.
	
	Assume that the claim holds for round $t_{i - 1} \leq t'$.
	Consider a node $u \not \in S$. 
	By definition, either $u$ does not beep at all in phase $q$, or it is super-heavy.
	In either case, we know the behavior of $u$ in round $t_{i - 1}$.
	The last case of $u \in S$ follows from the induction hypothesis.
	Recalling that the set $S$ contains all nodes that may join the MIS, we can check, in the end of the simulation of phase $[t, t']$, which nodes are removed from the graph.
\end{proof}









% Recursive beeping MIS algorithm.
% Input is node $u$, level $i$, and iteration $j$.

% \begin{definition}
% 	Node $v$ is called super-heavy in phase of length $2^i \cdot k$, if 
% \[
% 	d_{t_{i, j}}(v) \geq 2^{2^i \cdot 5k}
% \]
% \end{definition}


\begin{lemma}
	Consider some phase $[t, t']$ of length $2^i \cdot k$ and let $v$ be a node such that $d_{t}(v) < 2^{2^i \cdot 5k}$.
	For some $k = \bigO(\log \log \Delta)$, every node in $S_{[t, t']}(v)$ has at most $2^{2^i \cdot 8k}$ neighbors in $S_{[t, t']}(v)$ with probability at least $1/\Delta^{100}$.
	\label{lemma:ssize}
\end{lemma}
\begin{proof}
	Since super-heavy nodes are not added to the set $S$, we can assume for the worst case that $v$ has no super-heavy neighbors in phase $[t, t']$.

	In the worst case during the $2^{i} \cdot k$ rounds of phase $q$, the probability $p_t(u)$ to beep of all $u \in \nbh(v)$ doubles in every round of phase $q$.
	Thus, 
	\[
		d_{t}(v) \leq 2^{2^i \cdot 5k} \cdot 2^{2^i \cdot k} = 2^{2^i \cdot 6k} \ ,
	\]
	for every round $t$ of phase $q$. 
	Thus, the expected number of sum of beeps in the neighborhood of $v$ is at most 
	\[
		2^{2^i \cdot 6k} \cdot 2^i \cdot k \leq 2^{2^i \cdot 7k} \ .
	\]
	By applying a Chernoff bound, we get that, the number of beeps in the neighborhood of $v$ is more than $2^{1 + 2^i \cdot 7k} \leq 2^{2^i \cdot 8k}$ with probability at most
	\[
		\left( 2^{- \frac{2^i \cdot k}{3} } \right) \leq 2^{-\frac{k}{3}} \ .
	\]
	The lemma follows by setting $k \geq 300 \log \log \Delta$.
\end{proof}



% \begin{enumerate}
% 	\item The oracle $\orcG$ is able to simulate the fine-grained MIS up to round $t$.
% 	\item Measure $Q(\log \Delta / 2^i)$ describes how many queries are needed to simulate a phase of length $2^i \cdot k$ in a graph of max degree $2^{2^i \cdot 8k}$.
% \end{enumerate}

% \begin{definition}
% 	Let $O_{i, j}(v)$ be an oracle that answers whether node $v$ join the MIS in phase $j$ in level $i$ and if not, returns $p_{j + 1, i}^{*}(v)$ (if $j + 1 < 2^{i}$).
% \end{definition}







% In \cref{alg:oracle}, we give a pseudo-code representation of an implementation of an oracle, that simulates a phase $[t, t']$ of the fine-grained MIS algorithm.

% \begin{algorithm}
% 	\caption{Oracle for phase $[t_0, t_0 + 2^i \cdot k]$ for node $v$}
% 	\begin{algorithmic}
% 		\Require{Query access to the Oracle $\orcGt{t_0}$.}
% 		
% 		\State Set $t_1 = t_0 + 2^{i - 1} \cdot k - 1$.								\Comment{First iteration of the second subphase.}
% 		\State Set $t_2 = t_0 + 2^{i} \cdot k - 1$.									\Comment{First iteration of the next phase.}
% 		\State Obtain $p_{t_0}(u) = \orcGt{t_0}(u)$ for all $u \in N(v)$.			
% 		\State Set $d_{t_0}(v) = \sum_{u \in N(v)}$.
% 		
% 		\If{$d_{t_0}(u) \geq 2^{(\log \Delta) / 2^i}$}
% 			\State \Return $p_{t_0}(v) \cdot \frac{1}{2}^{(\log \Delta)/ 2^i}$ 			\Comment{super-heavy}
% 		\Else	
% 										
% 			\If{$i = 0$} 																	
% 				\State Simulate the beeping algorithm for $k$ iterations.				\Comment{Find all nodes in $S$.}
% 				\State \Return $p_{t_0 + k}(v)$
% 			\EndIf
% 		
% 			\If{$i > 0$} 
% 			
% 			\vspace{+3pt}
% 																
% 				\State Simulate phase $[t_0, t_1]$ and obtain $p_{t_1}(v)$.				\Comment{Create $\orcGt{t_1}$}	
% 				\State Simulate phase $[t_1, t_2]$ and obtain $p_{t_2}(v)$.
% 				\State \Return $p_{t_2}(v)$
% 			\EndIf
% 		\EndIf
% 	\end{algorithmic}
% 	\label{alg:oracle}
% \end{algorithm}

% \subsection{Oracle Wrapping\ju{this term sucks}{}}


% Let us define $Q([t, t'], \Delta_i)$ to be the query complexity needed to simulate $[t, t']$ on a graph $G_i$ with max degree $\Delta_i$, where each node $v$ is labeled with the value $p_t(v)$.

% \paragraph{Degree Bound. (= warm up to the idea in the next paragraph)}
% The keys to minimizing the number of queries made in the simulation are the two following observations.
% \begin{enumerate}
% 	\item Simulating phase $[t, t']$ for node $v$ in which $v$ is super-heavy, requires $\Delta$ queries to $\orcG$.
% 	\vspace{+3pt}
% 	\item If $v$ is not super-heavy, Lemma~\ref{lemma:ssize} promises that at most $2^{2^i \cdot 8k}$ neighbors of $v$ beep in this phase. The non-beeping neighbors of $v$ do not affect the behavior of $v$ in the phase and can be ignored for the simulation. 
% \end{enumerate}
% \textbf{Important: Notice that the delta factor denoted by a * comes from the fact that we need to query every node adjacent to the set $S$ with $\orcG$ to learn whether the $S$ nodes are super-heavy or not.}

% \paragraph{Trying to Argue How to Create $G_i$}
% What goes currently wrong:
% It is not enough to label nodes in $S$ with their $p_t(u)$ values! Instead, we need to label nodes in $N(S)$ so that we know how their beeps affect nodes in $S$.
% Important notice is, that we dont need to know what the neighbors of $N(S)$ do to know what nodes in $S$ do.

% We are finally ready to utilize the power of the LCA model in the simulation and show that our approach drops the query complexity significantly.
% The first step is to argue, why nodes executing a subphase $[t,2t]$ of phase $[t, 4t]$ for some $t > 0$ should have an access to the oracle $\orcG$ for free.
% Informally, one can think of it as follows.
% Whenever we wish to simulate the behavior of a node $u$ in subphase $[t, 2t]$, we must figure out whether $u$ is in $S_{[t, 2t]}$ or not.
% This can be accomplished by querying $\orcG$.
% If we do this automatically for every node we simulate, the simulation of subphase $[t, 2t]$ effectively takes place on a graph induced by $S_{[t, 2t]}$ which, in particular, has a smaller degree than $S_{[t, 4t]}$.
% Additionally, if we think of it as this ``automatic'' process, we can count the price of \emph{wrapping} the graph $G[S_{[t, 4t]}$ into a new graph $G[S_{[t, 2t]}]$ to the cost of the parent phase.

% Even better:
% We can do the very same thing for the phase $[2t + 1, 4t]$.
% In other words, we can run the simulation on a graph induced by nodes $S_{[t2 + 1, 4t]}$ and simply count the price of the wrapping as an cost factor of $\Delta \cdot Q(2t)$ in the parent phase.

% create oracle access to $S_{[t, 2t]}$ from $S_{[t, 4t]}$.\ju{what is this even supposed to mean?}
% This can be done by querying $\orcGt{[t, 4t]}(u)$ for all nodes and their neighbors in $S_{[t, 2t]}$, requiring $\Delta \cdot Q(S_{[t, 2t]})$ queries.
% The next step is to create access to the oracle $S_{[2t, t]}$

% \paragraph{Requirements}
% While the simulation is superficially quite clean, there are some less beautiful details hidden behind the scenes.
% To be really able to run the simulation of a phase $[t_1, t_2]$, we need to ensure the following when querying $\orc_{t_1}{t_2}(v)$.\ju{We dont even need anything else, right?}
% \begin{enumerate}
% 	\item The preparation phases are performed properly by the parent phase. More precisely, consider $[t_1, t_2]$ and $[t_2, t_3]$, that are subphases of phase $[t_1, t_3]$.
% 	\item Before calling either $\orc_{t_1, t_2}(v)$, or $\orc_{t_1, t_2}(v)$, we know $p_{t_t}(u)$ for all $u \in N(v)$. Otherwise, we cannot perform the preparation step of phase $[t_2, t_3]$.
% 	\item Is it clearer if we say that the graph needed to simulate stuff is known?
% \end{enumerate}

\subsection{Oracle Implementation}

\paragraph{Saving Queries.}
For the sake of an example, let as assume that for the simulation of any phase $[t, t']$, we have access to an oracle answering adjacency queries to the graph $\Gtt{t}{t'}$.
Let $\ell = t' - t$.
For the naive simulation of phase $[t, t']$ for node $v$, we need to learn the $(t' - t)$-hop neighborhood of $v$.
Given Lemma~\ref{lemma:ssize}, we get that at most $\left( 2^{8 \ell} \right)^{\ell} = 2^{8 \ell^2}$ queries are needed.
If we split the execution into two shorter subphases, the simulation becomes much more efficient.
Since the length of the subphases is roughly $\ell/2$, we get that the query complexity of the simulation drops to $2^{8 \ell/2} \cdot 2^{8 \ell/2} = 2^{8\ell}$, which is almost quadratically smaller.

Even though the above example cuts corners, we learn an important fact.
It is enough for us to reason how to (inductively) provide oracle access to graph $\Gtt{t}{t'/2 - 1}$ from oracle access to the graph $\Gtt{t}{t'}$.
Once we have access to $\Gtt{t}{t'/2 - 1}$, we can show how to combine these oracles to get access to $\Gtt{t'/2}{t'}$.

\paragraph{Creating the Oracles.}
Now, we finally go into implementing our oracles in more detail.
Our aim is to create an oracle that, for phase $q = [t, t']$ returns the neighbors of node $u$ in $G_{t, t'}$ and the $p_t(v)$ value.
Some notation follows
\begin{enumerate}
	\item We denote by $\orcGtt{t}{t'}$ the oracle that returns the adjacency list (in $\Gtt{t}{t'}$) and the $p_t(v)$ value of a query node $v$. For the sake of simplicity of notation, we often identify the oracle $\orcGtt{t}{t'}$ with the graph $\Gtt{t}{t'}$.
	\vspace{+3pt}
	\item We denote by $Q\left(\orcGtt{t}{t'}\right) = Q(\Gtt{t}{t'})$  an upper bound on the query complexity of a query to oracle $\Gtt{t}{t'}$.
	\vspace{+3pt}
	\item Furthermore, we denote the query complexity of simulating the phase $[t, t']$, given access to $\Gtt{t}{t'}$ by $Q([t, t'] \mid \Gtt{t}{t'})$. The maximum degree of $\Gtt{t}{t'}$ is denoted by $\Dtt{t}{t'}$.
\end{enumerate}

\begin{remark}
 To be precise, the adjacency oracle to $\orcGtt{t}{t'}$ needs to also return the $p_t(v)$ values of nodes in $N\left(S_{[t, t']}\right)$ for us to be able to use Lemma~\ref{lemma:correctness}.
 This condition is satisfied by the implementation of $\orcGtt{t}{t'}$ since it knows which nodes adjacent to the query node $v$ are super-heavy or do not beep.
 We leave this property out of our notation to avoid making it more cluttered and just assume it implicitly. 
\end{remark}

Consider now $\orcGtt{0}{T}$, where $T \in \bigO(\log \Delta + \log(1/\eps))$ is the runtime of the \algo{} algorithm.
Assume w.l.o.g., that $T = 2^i \cdot k$ for some $i \geq 0$.
Clearly, the adjacency oracle $\orc^G$ of the input graph satisfies the properties required by $\orcGtt{0}{T}$.
Then, by induction and by Lemma~\ref{lemma:overhead}, we get a construction for an adjacency oracle $\orcGtt{t}{t'}$ for any graph $\Gtt{t}{t'}$.

% Each such oracle is created inductively from the corresponding oracle of the parent phase.

% Assume then that we have obtained oracle $\orcGtt{t}{t'}$ for some $t' - t > k$, i.e., phase $[t, t']$ can be divided into two subphases.



% \begin{definition}
% 	Let $Q([t, t'] \mid \Gtt{t}{t'})$ denote the number of queries needed to simulate phase $[t, t']$ given a free access to $\orcGtt{t}{t'}$.
% \end{definition}



\begin{lemma}
	Assume that there is an adjacency oracle for the graph $\Gtt{t}{t'}$.
	Then, an adjacency query access to the graph $\Gtt{t}{t'/2 - 1}$ can be implemented with $Q(\Gtt{t}{t'})$ queries.
	Furthermore, an adjacency query access to the graph $\Gtt{t'/2}{t'}$ can be implemented with $Q(\Gtt{t}{t'}) \cdot  Q([t, t'/2 - 1] \mid \Gtt{t}{t'/2 - 1} )$ queries and the whole simulation of phase $[t, t']$ requires $\Dtt{t}{t'} \cdot  Q([t, t'/2 - 1] \mid \Gtt{t}{t'/2 - 1} ) \cdot Q([t'/2, t'] \mid \Gtt{t'/2}{t'} )$ queries.
	\label{lemma:overhead}
\end{lemma}
\begin{proof}
	Let $v$ be a node that we wish to simulate in phase $[t, t']$.
% 	By setting $\Gtt{t'/2}{t'} = S_{[t'/2, t']}(v)$, the measure $Q( [t, t'/2 - 1] \mid Q(\Gtt{t'/2}{t'}) )$ is exactly the number of queries needed
	To simulate the behavior of $v$ in the subphase $[t'/2, t']$, we require $Q([t'/2, t'] \mid \Gtt{t'/2}{t'} )$ adjacency queries to graph $\Gtt{t'/2}{t'}$.
	For each of these queries to some node $u$, we need to simulate the behavior of the queried node $u$ in phase $[t, t'/2 - 1]$.
	This simulation of $u$ requires $Q([t, t'/2 - 1] \mid \Gtt{t}{t'/2 - 1} )$ queries.
	Finally, to perform an adjacency query of node $u$ in $\Gtt{t}{t'/2 - 1}$, we need to query all the $\Dtt{t}{t'}$ neighbors of $u$ in the graph $\Gtt{t}{t'}$ to learn which of these nodes are actually part of $\Gtt{t}{t'/2 - 1}$.
	Thus, the number of queries needed to simulate phase $[t, t']$ adds up to
	\[
		Q([t, t'] \mid \Gtt{t}{t'}) = \Dtt{t}{t'} \cdot Q([t, t'/2 - 1] \mid \Gtt{t}{t'/2 - 1}) \cdot  Q([t'/2, t'] \mid \Gtt{t'/2}{t'} ) \ . \qedhere
	\]
\end{proof}

% \begin{observation}
% 	$Q([t, t'] \mid \Gtt{t}{t'}) = Q([t, t'/2 - 1] \mid \Gtt{t}{t'/2 - 1}) \cdot Q([t'/2, t'] \mid \Gtt{t'/2}{t'})$.
% 	\label{obs:saving}
% \end{observation}
% Essentially, Observation~\ref{obs:saving} says that the price of simulating phase $[t, t']$ can be split into two parts corresponding to the subphase if we are given an oracle access to the graphs in which the phases are executed.
% The crucial thing here is, that graphs $\Gtt{t}{t'/2 - 1}$ and $\Gtt{t'/2}{t'}$ have a much smaller degree than $\Gtt{t}{t'}$.
% Let us identify $\Gtt{t}{t'}$ with $S([t, t'])$ and similarly for $S([t, t'/2 - 1])$ and $S([t'/2, t'])$ and let $\Delta_{t, t'}, \Delta_{t, t'/2 - 1},$ and $\Delta{t'/2, t'}$ be an upper bound on the maximum degree of  $\Gtt{t}{t'/2 - 1}$, $\Gtt{t'/2}{t'}$, and $\Gtt{t}{t'}$, respectively.
% Writing $t' - t = 2^i \cdot k$ for some $i$, we get by Lemma~\ref{lemma:ssize} that 
% \[
% 	\max\{ \Delta_{t, t'/2 - 1}, \Delta_{t'/2, t'} \} \leq 2^{2^{i - 1} \cdot 8k} \ll \Delta_{t, t'} \leq 2^{2^{i} \cdot 8k}  \ .
% \]\ju{write this correctly, i.e., stating that these are just the upper bound guarantees}

% Therefore, what remains to do is to show how to obtain access to queries to the graphs $\Gtt{t}{t'/2 - 1}$ and $\Gtt{t'/2}{t'}$ using access to $\Gtt{t}{t'}$.
% Access to $\Gtt{t}{t'/2 - 1}$ is straightforward.
% For query $\Gtt{t}{t'/2 - 1}(u)$, we need to execute queries to all $\Gtt{t}{t'}(w)$, where $w$ is a neighbor of $u$ in graph $\Gtt{t}{t'}$.







\begin{lemma}
	Let $k \geq 300\log \log \Delta$ and recall that a block is a phase of length $k$.
	The size of $S_{[t, t']}(v)$ for some block $[t, t']$ of node $v$ is $\Delta^{\frac{\bigO(\log^2 \log \Delta)}{\log \Delta}}$. 
	\label{lemma:baseComplexity}
\end{lemma}
\begin{proof}
	Since the length of a block is $k$, we get by Lemma~\ref{lemma:ssize} that the size of $S_{[t, t']}(v)$ is, with probability at least $1/\Delta^{100}$, bounded from above by
	\[
		\left( 2^{8k} \right)^{k} = 2^{8k^2} \leq 2^{\bigO(\log^2 \log \Delta)} = \Delta^{\frac{\bigO(\log^2 \log \Delta)}{\log \Delta}} = \Delta^{o(1)} \ . \qedhere
	\]
\end{proof}

% \begin{lemma}
% 	Given a free query access to $\orcG$, simulating phase $[t, t']$ of length $2^i \cdot k$ of node $v$ requires $\Delta \cdot Q((\log \Delta)/2) \cdot Q((\log \Delta)/2^i)$ queries.
% 	\label{lemma:numqueries}
% \end{lemma}
% \begin{proof}
% 	Let $Q((\log \Delta)/2^i)$ be defined as the number of nodes that are involved in phase $[t, t']$ of node $v$.
% 	A query to $\orcGt{t + 2^{i - 1} \cdot k}$ can be implemented with $\Delta \cdot Q((\log \Delta)/2^i)$ queries.
% 	Thus, we need $\Delta \cdot Q((\log \Delta)/2^i) \cdot Q((\log \Delta)/2^i)$ queries in total.
% \end{proof}

\begin{theorem}
	The query complexity of simulating the \algo{} algorithm is bounded from above by $\Delta^{\bigO(\log \log \Delta)}$.
	\label{thm:numqueries}
\end{theorem}
\begin{proof}
	Let $T = \bigO(\log \Delta + \log(1/\eps))$ for some $\eps > 0$ needed to get the shattering guarantee by Lemma~\ref{lemma:shattering}.
	Assume w.l.o.g., that $T = 2^\ell \cdot k$ for some integer $\ell \geq 0$, where $k$ is the length of a block.
	To make the rest of the proof readable, let us abuse our notation a bit and, for phase $[t, t']$ of length $T/2^i$, denote by $Q(T/2^i) = Q([t, t'] \mid \Gtt_{t}{t'})$ an upper bound on the query complexity, over all phases of length $T/2^i$.
	Let us also use a shorthand $\Dt{T/2^{i}} = \Dtt{t}{t'}$ to denote the maximum degree of $\Gtt{t}{t'}$.	
	By Lemma~\ref{lemma:overhead} and Lemma~\ref{lemma:ssize}, we can write the query complexity of phase $[t, t']$, where $t' - t > k$, as
	\begin{align*}
		Q(T/2^i \mid \Gtt{t}{t'}) 	& = Q(T/2^i) = \Dt{T/2^i} \cdot Q(T/2^{i + 1}) \cdot Q(T/2^{i + 1}) \\
									& = 2^{2^i \cdot 8k} \cdot Q(T/2^{i + 1}) \cdot Q(T/2^{i + 1}) = 2^{2^i \cdot 8k} \cdot Q(T/2^{i + 1})^2 \ .
	\end{align*}
	
	By Lemma~\ref{lemma:overhead} and Lemma~\ref{lemma:baseComplexity}, we get the following recursion.
	\begin{align*}
		Q([1, T], G) & = \Dtt{1}{T} \cdot Q(T/2) \cdot Q(T/2) = \Dtt{1}{T} \cdot Q(T/2)^2 \\
					%= \Dt{T} \cdot \left(\Dt{T/2} \right)^2 \cdot Q(T/4)^4 = \ldots \\		
					 %
					 & = \Dt{T} \cdot \left(\Dt{T/2} \right)^2 \cdot Q(T/4)^4 = \ldots \\					 
					 %
					 & = \Dt{T} \cdot \left( \Dt{T/2} \right)^2 \cdot \ldots \cdot 2^{\bigO(\log \log \Delta)} \cdot Q(\log \log \Delta)^{\frac{\log \Delta}{\log \log \Delta}}\\
					 %
					 & = 2^{\left( \sum_{i = 1}^{\log T} 2^i \cdot 8k \right)} \cdot \left( \Delta^{\frac{\bigO(\log^2 \log \Delta)}{\log \Delta}} \right)^{{\frac{\log \Delta}{\log \log \Delta}}} = 2^{\bigO( \log \Delta \cdot \log \log \Delta )} \cdot \Delta^{\bigO(\log \log \Delta)} \\
					 %
					 & = \Delta^{\bigO(\log \log \Delta)} \cdot \Delta^{\bigO(\log \log \Delta)} = \Delta^{\bigO(\log \log \Delta)} \ .  \qedhere
	\end{align*}
\end{proof}

\section{Post-Shattering}
In this section, we do some clean up work and show how Theorem~\ref{thm:numqueries} leads to the proof of Theorem~\ref{thm:main}.
A careful reader may have noticed that there are two small discrepancies between our simulation and the \algo{} algorithm.
Next, we explain what these discrepancies are and how to deal with them.

\paragraph{Removing Nodes in the End of Simulation of a Phase.}
To be precise, Lemma~\ref{lemma:correctness} only guarantees that a node $v \not \in S$ knows in the \emph{end} of phase $[t, t']$ whether it joined the MIS or not.
In the \algo{} algorithm, removal of the MIS nodes happens after every round.
From the perspective of the nodes that are not in $S$ because they do not beep in the whole phase, there is no difference.
A careful look at the analysis of \algo{} algorithm shows that it is robust against late removals of super-heavy nodes as well.
In particular, Lemma~\ref{lemma:sparse} and Lemma~\ref{lemma:dense} are not affected by super-heavy neighbors.
Furthermore, the statements in Lemma~\ref{lemma:runtime} do not differentiate between the cases where neighbors get removed or not.


\paragraph{Nodes with too many Neighbors in $S$.}
In Lemma~\ref{lemma:ssize}, we state that the number of neighbors of any node in $S$ that are in the set $S$---i.e., the degree of the node in the subgraph induced by $S$---is bounded.
However, this claim ``only'' holds with high probability (i.e., $1/\Delta^{100}$).
We can unify the simulation and the \algo{} algorithm by adding a check into the \algo{} algorithm, so that we remove a vertex from the graph (to be dealt with after the shattering) if this high probability event is violated.
For Theorem~\ref{thm:beeping}, we only require that the probability of a vertex surviving the \algo{} algorithm is polynomially small in $\Delta$ and thus, the claim still holds.




\paragraph{Small Components.}
Once the simulation of the \algo{} algorithm is complete, we get the shattering guarantee from Lemma~\ref{lemma:shattering}.
In other words, we are left with polylogarithmic size components of the input graph.
To finish off our algorithm, we simply query all of these nodes in a brute-force fashion and find an arbitrary MIS.
This requires at most an additional factor $\bigO(\log n \cdot \Delta^4)$ in the query complexity, yielding Theorem~\ref{thm:main}.







% }

% \paragraph{Cheating}
% Notice that we are cheating a bit in \cref{alg:oracle}. The oracle $\oracle{i}{j - 1}$ that is called in the recursion is only implemented implicitly.
% Essentially, the caller of $\oracle{i}{j}$ already must know this value due to earlier queries.
% The algorithm is just less cluttered this way.
% Actually, this cheating step seems to be the most important.
% We lose information when nodes are super-heavy:
% If node $v$ is super-heavy in phase $(i, j)$, then we do not simulate its neighbors in this phase.
% Therefore, when we go to phase $(i, j + 1)$, we need to do this simulation.
% It gets uglier:
% All the $Q(\Delta/2^i)$ nodes ``opened up'' this way might have to be simulated to figure out $p_{i, j + 2}$.

% \begin{algorithm}
% 	\label{alg:oracle}
% 	\caption{$\oracle{i}{j}(u, p_{j \cdot 2^i}(u))$}
% 	\begin{algorithmic}
% 		\State Set $\ell = j \cdot 2^i$.												\Comment{Shorthand for the current iteration.}
% 		\If{$i = 0$} 																	\Comment{Base case}
% 			\State For all $u \in N^{k}(v)$, obtain $p_{\ell}(u)$.
% 			\State Simulate the beeping algorithm for $k$ iterations.					\Comment{$\Delta^{k}$ queries}
% 			\State \Return $p_{\ell + k}(u)$.
% 		\EndIf
% 		
% 		\If{$i > 0$} 
% 			\State Obtain $p_{\ell}(v) = \oracle{i - 1}{j}(v)$ for all neighbors $v$ of $u$.

% 			\State Let $d_{\ell}(u) = \sum_{u \in N(v)} p_{\ell}(v) = \sum_{u \in N(v)} \oracle{i}{j}(v)$.
% 			\vspace{+3pt}

% 			\If{$d_{\ell}(u) \geq 2^{(\log \Delta) / \ell}$}
% 				\State \Return $p_{\ell}(u) \cdot \frac{1}{2}^{(\log \Delta)/{\ell}}$ 	\Comment{super-heavy}
% 			\Else
% 				\State Obtain $p_{\ell}(u) = \oracle{i + 1}{2j}(u)$.					\Comment{Recursive call to next level}
% 			\EndIf
% 			
% 			\State Obtain $p_{\ell}(v) = \oracle{i}{j}(v)$ for all neighbors $v$ of $u$.				
% 			\If{$d_{\ell}(u) \geq 2^{(\log \Delta) / \ell}$} 
% 				\State \Return $p_{\ell}(u) \cdot \frac{1}{2}^{(\log \Delta)/{\ell}}$	\Comment{super-heavy}			
% 			\Else
% 				\State \Return $\oracle{i + 1}{2j + 1}(u)$								\Comment{Recursive call to next level}
% 			\EndIf
% 		\EndIf
% 	\end{algorithmic}
% \end{algorithm}


% \spotlight{Consider a node $v$ that is \textbf{not} super-heavy. This implies that many neighbors have to be relatively light. 
% Since the sum of the beeping probabilities of the light neighbors is small, it implies that many of them will not beep at all in the current phase.
% The behavior of such nodes is trivial to simulate.}


% \section{Fine Grained MIS}




% Effectively, the whole execution of the algorithm can be thought of as a very long phase of $\bigO( \log \Delta )$ rounds.
% The above section essentially divides this phase into many, with a parameter $\mu = \sqrt{\log \Delta}$ of desired number of subphases.
% This, in turn introduces the parameter that defines the super-heavy nodes, i.e., the nodes that do not join the MIS during the subphase.

% More generally, we can do the same trick with any $2 \leq \mu = o(\log \Delta)$.
% Then, a super-heavy node is a node with $d_{t_i} \geq 2^{(\log \Delta) / (10\mu)}$.
% In other words, a super-heavy node will not be chosen to the MIS during this subphase.

% For example, by setting $\mu = 2$, we can exclude nodes who have no chance in getting into the MIS during the first half of the execution of the beeping algorithm.
% Then, we can divide this new subphase, where some nodes are already excluded, further into two subphases and exclude super-heavy nodes that have no chance of entering the MIS and so on.
% In addition, we examine the light nodes in an analogous way to the previous section.
% Let $T = \bigO(\log \Delta)$ be the runtime of the beeping algorithm.
% Recursing all the way to constant length subphases, we end up simulating $\log T$ subphases of constant length.

% \paragraph{Keep in Mind.}
% A thing to keep in mind is that simulating a constant length subphase does not (necessarily at least) work with $\bigO(1)$ queries.
% To simulate a short subphase, we may end up querying all neighbors at least once\ju{Perhaps one can save some queries by only looking at nodes that actually beep in a short subphase. Especially, if we start with probabilities larger than $1/2$ and show that we stay around $d(u) = \log \Delta$ with high probability.}.
% Plugging this into the recursion yields a factor of $\Delta$ in front of every recursive call.
% Thus, we require $\Delta^{\log T} = 2^{\log \Delta \cdot \log \log \Delta}$ queries. 

% Another thing to keep in mind is that an oracle that simulates a node $v$ does not need to know the outcomes of the currently simulated phase of other nodes.
% For example:
% A super heavy neighbor can just be assumed to beep in every step. Analysis goes through. Notice though that this can be ``pessimistic'' in the sense that node $v$ could join the MIS if a super-heavy node was removed and does not beep when the beep vector indicates so.
% A node that does not beep at all, will not affect anything. The behavior of this node may affect future phases,  but that is to be cared about when creating oracles for future phases.


% \newpage
% \paragraph{Old Exercise}
% As an exercise, let us first consider a simplified case, where the execution consists of one phase of length $2^2 \cdot k$, i.e., the execution gets divided into two subphases and four blocks.
% For the purpose of this toy example, assume that either node $v$ is super-heavy, or the maximum number of neighbors of $v$ that beep in a phase of length $2^i \cdot k$ is bounded by $2^{(2^2 \cdot k) / 2^i}$, for $i \in \{1, 2\}$.
% Later, we will use \cref{lemma:sparsenbh} to obtain a similar restriction in our real simulation.

% Our aim is to create an oracle access, through oracle $\orc$, to the input graph that, given a node $v$ and a phase, returns the $p_t(v)$ value in the end of that phase.
% In other words, $\orc$ performs all the queries needed to simulate the actions of the nodes that can influence the $p_t(v)$ value.
% Let us consider the second phase of length $2 \cdot k$, denoted by $q_2$ and $q_1$ is defined similarly.
% There two important observations to take into account
% \begin{enumerate}
% 	\item	Let $t$ be the first round of $q$. Oracle $\orcG$ knows $p_t(v)$ before any queries need to be made.
% 	\item	Since $q_2$ was initiated by the parent phase, we have to know $p_t'(u)$ for all $u \in N(v)$, where $t'$ is the first round of $q_2$.
% \end{enumerate}

% \paragraph{Preparation Step}
% To implement the oracle that simulates this phase, our first task is to learn what are the $p_t(u)$ values for all neighbors $u$ of $v$, where $t$ is the first round of this phase.
% This involves simulating phase $q_2$ of length $2 \cdot k$ for all neighbors of $v$, requiring 
% \[
% 	\Delta \cdot Q(\log \Delta/4) \cdot Q(\log \Delta/4) = 2^{2^2 \cdot k} \cdot 2^{(2^2 \cdot k)/4 + (2^2 \cdot k)/4 + 2} = 2^{2^2 \cdot k + k + 2} \ .
% \]
% Notice that the recursive query produces additive terms in the exponent, implying that the query complexity grows linearly with the recursion depth.
% As the second step, we can just do the simulation by querying $v$.
% To put down the whole complexity, we get
% \[
% 	Q(\log \Delta) = \Delta \cdot Q(\log \Delta / 2) \cdot Q(\log \Delta / 2) = \Delta^{3} \cdot Q(\log \Delta / 2)^4 = 2^{3 \cdot 2^2 \cdot k + 4k} = 2^{\bigO(k)} \ .
% \]













==> model.tex <==
We consider Local Computation Algorithms (LCA).
The model is roughly as follows:
\begin{enumerate}
	\item Initially, there is an unknown graph $G = (V ,E)$. We are given access to a query oracle that answers node queries with the neighborhood of the corresponding node.
	\item The algorithm has access to a string of random bits. This can be viewed as a vector of random bits for every node. In particular, every node ``knows'' the random bits of the other nodes (when we think about simulating distributed algorithms).
	\item We sequentially query the oracle and learn neighborhoods of nodes. A local computation algorithm remembers the whole history.
	\item For a node $v \in V$, the output is whether the node is in the MIS or not.
	\item The running time is the maximum number of queries for any node and thus, every distributed algorithm can be simulated in $\bigO\left( \Delta^{T(n)} \right)$ time, where $\Delta$ is the maximum degree and $T(n)$ the runtime of the distributed algorithm.
\end{enumerate}

Any LCA algorithm is given access to a string of random bits.
Assuming the knowledge of the number of nodes $n$ and that every node is assigned a unique identifier
This implies, that once node $u$ is queried and we learn the identifiers of its neighbors, we also learn all the randomness that these nodes use in the execution.

We study the MIS problem in the aforementioned model.
The goal is to achieve a runtime of roughly polynomial in $\Delta$ and, more precisely, $2^{\log^{1 + \epsilon} \Delta}$ for some small $\epsilon > 0$.

\newpage

==> sketch.tex <==
The basic idea is to simulate the $\sqrt{\log \Delta}$-round CONGESTED CLIQUE algorithm (say $A$) from the ``Distributed MIS via All-to-All Communication'' -paper~\cite{Ghaffari2017}.
In their paper, the take a $\bigO(\log \Delta)$ time MIS algorithm in the CONGEST model and transform it into a $\sqrt{\log \Delta}$-round CC algorithm.

\subsection{The Straightforward and Slow Way}
The canonical way to simulate the algorithm is as follows.
For any node $v$, learn the $k$-hop neighborhood of $v$, where $k$ is the maximum distance from $v$ to any node that influences the decision of $v$ according to $A$.
The annoying thing is that there might be nodes in distance roughly $\log \Delta$ that influence the decision of $v$.
Thus, we may have to query $\Delta^{\log \Delta}$ nodes.

\subsection{Do Not Query All Nodes}
In the paper by Ghaffari, they employ a beeping style MIS algorithm, where every node beeps with some probability in every round and if the node beeps alone, it joins the MIS.
The probabilities of the beeps are dynamically adjusted depending on whether there is a collision of beeps or if no one in the neighborhood beeps.

The trick is roughly speaking to observe that the execution of this beeping algorithm can be divided into three cases.
\begin{enumerate}
	\item {\bf The good case.} Node $v$ enters the MIS with a constant probability.
	\item {\bf Super heavy.} The probability of at least one node in $\nbh(v)$ to beep is at least $2^{\sqrt{\log \Delta}}$. In this case, we can assume that there is always a neighbor of $v$ who beeps. Furthermore, this property holds for roughly the following $\sqrt{\log \Delta}$ rounds.
Node $v$
	\item {\bf Light.} The probability of some node in the neighborhood to beep is very small. In this case, we know that the probabilities to join the MIS will go up fast.
\end{enumerate}

For our purposes it is convenient to think of the neighborhood of a node $u$ as a tree rooted at $u$. 
We can effectively assume that the local neighborhood of $u$ is a tree, since this is the case where querying the neighborhood is the most expensive, i.e., every neighbor of every node has to be queried individually.

To avoid a runtime exponential in $\Delta$, we try to avoid querying nodes that are irrelevant for some phase.
These nodes correspond to the super heavy nodes described above.
Since these nodes will not join the MIS in the phase, it is not necessary to simulate them nor their children of these nodes in the current phase. 
This way, we are able to (locally) sparsify the graph such that any node $v$ only has to learn about of roughly $\sqrt{\log \Delta}$ nodes in its $\bigO(\log \Delta)$-neighborhood.

















==> sparseMIS.tex <==
This section just repeats the algorithm from~\cite{Ghaffari2017}.
It might be convenient to have this here for reference.



The algorithm works in phases, each made of $P = \sqrt{\log \Delta}/10$ iterations and one additional round.
At the beginning of each phase, before the iterations, we have one round where each node $v$ sends its $p_t(v)$ to its neighbors.
Initially, $p_1(u) = 1/2$.

\begin{definition}
	The local density in round $t$ is defined as $d_t(u) = \sum_{v \in \nbh(u)} p_t(v)$.
\end{definition}

Let $t_i$ be the first round of phase $i$.
\begin{definition}
	A node is called \emph{super heavy} in phase $i$ if $d_{t_i}(v) \geq 2^{\sqrt{\log \Delta}/5}$.
\end{definition}

The algorithm then proceeds in iterations, each consisting of two rounds:
\begin{itemize}
	\item[(R1)] In the first round of iteration $t$, node $v$ beeps with probability $p_t(v)$ and remains silent otherwise.
				Node $v$ joins the MIS if the following three conditions are satisfied: $(1)$ Node $v$ is not super-heavy, $(2)$ node $v$ beeps, and $(3)$ none of the neighbors of $v$ beep. Node $v$ updates its beeping probability for the next iterations as follows:
				\[
					p_{t + 1}(v) = \begin{cases}
										p_t(v)/2, \text{if $v$ is super-heavy, or if at least one neighbor beeped.}\\
										\min{\{ 2p_{t}(v), 1/2\}}, \text{otherwise.}										
								   \end{cases}
				\]
				
	\item[(R2)] In the second round of iteration $t$, all nodes in the MIS beep. If a node not in the MIS hears a beep, it learns that it has an MIS neighbor. MIS nodes and their non-super-heavy neighbors get removed from the graph.
\end{itemize}



%Finally, in the end of each phase, we remove the super-heavy nodes from the graph that obtained an MIS neighbor.

The following theorem shows that in the local (or just beeping) model of computing, the algorithm terminates quickly.\ju{We can probably ignore R2 in the LCA simulation.}

\begin{theorem}[\cite{Ghaffari2017} ]
	\label{thm:beepruntime}
	For each node $v$, during $T = \bigO(\log \deg(v) + \log 1/\eps)$ rounds, where $C$ is a large enough constant, with probability at least $1 - \eps$, either node $v$ or a neighbor of node $v$ is added to the MIS. Furthermore, this guarantee holds independent of the randomness outside $2$-hop neighborhood of $v$.
\end{theorem}

==> sqrtn.tex <==
\section{Random Old Stuff}
% Similarly to \cref{lemma:sparse}, we get that for a node that is not super-heavy, the number of neighbors that beep in this phase is bounded by a polynomial of the length of the phase, i.e., $2^{1 + (\log \Delta)/8}$\ju{check} for the case of level $2$.
\begin{lemma}
	\label{lemma:generalSparse}
	Let $v$ such that $\log \Delta \leq d_{i, j}^{*}(v) < 2^{ (\log \Delta) / 2^{i - 1}}$.\ju{Whp doesnt hold anymore if density is below $\log \Delta$?}
	Then, with high probability, at most 
	\[
		2^{1 + (\log \Delta)/(2^{i}/2)} = 2^{(\log \Delta)/2^{i - 1}}
	\]
	neighbors of $v$ beep in phase $j$ of level $i$.
\end{lemma}
\begin{proof}
	In the worst case, $d(v)$ doubles in every round.
	Since the duration of phase $j$ of level $i$ is $2^{-i} \log \Delta$, we get that 
\[
	d_{i, j}(v) \leq  2^{(\log \Delta) / 2^i} \cdot 2^{ (\log \Delta) / 2^{i - 1}} \leq 2^{\log \Delta / 2^{i + 2}} = \Delta^{\frac{1}{2^{i + 2}}} 
\]
for the whole duration of the phase.
Thus, no more than 
\[
	2 \cdot \left( \Delta^{2^{-i - 2}} \right) \cdot 2^{-i} \log \Delta \leq \Delta^{ \frac{1}{2^{i - 1} } }
\]
neighbors of $v$ beep with high probability during the whole phase.



	Sanity check:
	\begin{enumerate}
		\item in the first phase, we have at most roughly $2^{\log \Delta / \bigO(1)} = \Delta$ neighbors beeping. Careful.
		\item If $i = \log \sqrt{\log \Delta} + 1$, then threshold for super-heavy is $2^{(\log \Delta) / 2^{\log \sqrt{\log \Delta} + 1 - 1}} = 2^{\sqrt{\log \Delta}}$.
		\item At most $2^{1 + (\log \Delta) / ( 2^{\log \sqrt{\Delta} + 1 - 1} )} = 2^{1 + (\log \Delta) / \sqrt{\log \Delta}} = 2^{1 + \sqrt{\log \Delta}}$ nodes beep.
	\end{enumerate}
\end{proof}

\begin{lemma}
	For any $j$, to implement $O_{\log \log \Delta, j}$, node $v$ needs to query $\Delta^{\bigO(1)}$.  neighbors.
\end{lemma}
\begin{proof}
Trololo

	\begin{itemize}
		\item 	Important: Threshold to the power of length is poly delta, for some constant exponent. This way, oracle in every recursion level takes poly delta time to simulate and results in Delta to poly log log Delta time in total (for poly log log recursion levels).
		\item	Length: $\log \Delta / 2^i$
		\item	Threshold: $2^{\log \Delta / 2^i}$
		\item	Expanding factor $ \Delta^{\frac{1}{2^{i - 1}}}$ beeping neighbors.
		\item	Need to query. This still sounds like too much.
				\[
					\left( \Delta^{\frac{1}{2^{i - 1}}} \right)^{\left( (\log \Delta)/2^{i} \right)}
				\]
		\item	If $i = \log \log \Delta$, then $2^{2i - 1} = (1/2) \cdot \log^2 \Delta$. Something is weird.. Now it looks like I could just split the whole execution into very short (constant length) phases and simulate those.
	\end{itemize}	

\end{proof}


\section{Simulating a Phase}
As a warm-up, let us assume that every node is labeled with their state in the beginning of some phase $i$, i.e., $p_{t_0}(u)$ for node $u$ is learned immediately when querying any neighbor of $u$.
% For more intuitive description, let us also assume that the local neighborhood of node $v$, whose output is to be inferred, is a tree.
% Notice that this is anyway essentially the worst case, since tree-like neighborhood maximizes the queries needed to learn it.
Our goal is to simulate phase $i$ for node $v$, i.e., learn whether node $v$ or one of its neighbors join the MIS and if not, what is $p_{t_{i + 1}}(v)$ of phase $i + 1$.

\spotlight{Consider the case where $v$ is super-heavy in phase $i$.
Unless some neighbor of $v$ joins the MIS in phase $i$, we can simulate the behavior of $v$ without considering the beeps of the neighbors.
In case a neighbor joins the MIS, we can stop the simulation.
}

%To check whether a neighbor joins the MIS, it is sufficient to simulate the non-super-heavy neighbors of $u$.}
%\ju{Notice here that I do not care about $p_{t_{i + 1}}(u)$. But I do need to know whether $u$ stops beeping due to a neighbor joining the MIS.} 


Let us shift our focus to nodes that are not super-heavy.
Now, we need to know the behavior of all the neighbors, regardless of their local density.
First, let us recall that by knowing the neighbors of $v$ from querying $v$, we know the random bit vector that determines whether they beep or not.

\spotlight{Since the local density of $v$ is relatively small, it has to be the case that there are many neighbors $u$ with a small $p_{t_0}(u)$. 
Therefore, there has to be many neighbors of $v$ who only toss coins that show tails.
For these nodes, there is no need to query any more nodes in their neighborhoods.
}

\begin{lemma}[Lemma 12~\cite{Ghaffari2017}]
% 	\label{lemma:sparse}
	Let $v$ such that $d(v) < 2^{\sqrt{\log \Delta} / 5}$ in the beginning of phase $i$.
	Then, with high probability, at most $2^{1 + \sqrt{\log \Delta}/2}$ neighbors of $v$ beep in phase $i$.
\end{lemma}
\begin{proof}
	In the worst case during the $\sqrt{\log \Delta}/10$ rounds of phase $i$, the probability $p_t(u)$ to beep of all $u \in \nbh(v)$ doubles in every round $t$ of phase $i$.
	Thus, 
	\[
		d_t(v) \leq 2^{\sqrt{\log \Delta} / 5} \cdot 2^{\sqrt{\log \Delta} / 10} = 2^{\sqrt{\log \Delta} \cdot \frac{3}{10}} \ ,
	\]
	for every round $t$ of phase $i$. 
	In other words, the expected number of sum of beeps in the neighborhood of $v$ is at most 
	\[
		2^{\sqrt{\log \Delta} \cdot \frac{3}{10}} \cdot 2^{\sqrt{\log \Delta} / 10} \leq 2^{\sqrt{\log \Delta} / 2} \ .
	\]
	By applying a Chernoff bound, we get that the number of beeps in the neighborhood of $v$ is $2^{1 + \sqrt{\log \Delta} / 2}$ with high probability\ju{whp in $\Delta$}.	
\end{proof}

\cref{lemma:sparse} essentially states that for a light node, there are many nodes in its neighborhood that will not beep in phase $i$ and can therefore be omitted from simulating this phase.
Another case that we have to consider is the case where a two-hop neighbor of $v$ enters the MIS. 
This can potentially change the behavior of a neighbor of $v$ and thereby, influence the value of $p_{t_{i + 1}}(v)$.
Since we simulate the full behavior of light of non-super-heavy nodes, the only case where this has influence is the case where a super-heavy neighbor of $v$ is kicked out of the graph.
However, this event can only increase the chance of node $v$ being removed from the graph during phase $i$, we simply ignore this possibility and do the removals of super-heavy neighbors of $v$ in the end of the current phase.\ju{Mohsen's analysis allows for this.}


We are now ready to describe the simulation of phase $i$.
To select which nodes to query, consider the following branching process.
Recall that we assumed for simplicity, that we learn $p_{t_i}(u)$ for any queried node.
We start from node $v$ and query all of its neighbors.

Every super-heavy neighbor beeps according to their respective random bits for phase $i$.
For every queried node $u$ that is not super-heavy, we recursively query all neighbors of $u$ that beep at least once during phase $i$.
Since the phase takes exactly $\sqrt{\log \Delta} / 10$ rounds, we have to query at most up to distance $\sqrt{\log \Delta} / 10$ from $v$.
Therefore, the number of nodes we must query is bounded from above by 
\begin{align}
	\left(2^{1 + \sqrt{\log \Delta} / 2} \right)^{\sqrt{\log \Delta} / 10} 
	& = 2^{\sqrt{\log \Delta} / 10 + (\log \Delta) / 20} \\ 
	& \leq 2^{(\log \Delta) / 10} = \Delta^{\frac{1}{10}} \ .
\end{align}

In essence, we have constructed an oracle $O_i$, that tells us whether node $u$ joined the MIS by phase $i$ or, if not, the probability $p_{t_i}(u)$.
Earlier, we assumed that every node $u$ knows the value $p_{t_i}(u)$ in the beginning of simulation of phase $i$.
We can obtain this inductively as follows.\ju{this seems rather trivial.}
We know that $p_{t_0}(u) = 1/2$ and therefore, the claim holds for the first phase.
From the simulation of phase $i$, we learn $p_{t_{i + 1}}(u)$ for any $u$.

\begin{lemma}
	\label{lemma:learn}
	Oracle $O_{i}$ can be implemented with a query complexity of $\Delta^{3i}$.
\end{lemma}
\begin{proof}
	The proof goes by induction on the phases.
	For the base case, consider phase $0$.
	In this phase, the probability $p_{0}(u) = 1/2$ for each node $u$, i.e., we know whether a node is heavy or light by learning the number of neighbors it has.
	In other words, for some node $v$, we learn the local densities of all $u \in \nbh(v)$ with $\Delta$ queries.
	Recalling that the beeps of super-heavy neighbors can be simulated without querying their neighbors and by \cref{lemma:sparse}\ju{probably make a more explicit lemma for this reference.}, we get that at most $\Delta + \Delta^{1/10}$ nodes have to be queried in the first phase, i.e., $O_0$ can be implemented with $\Delta + \Delta^{1/10}$ queries.
	
	Assume now that with $\Delta^{3j}$ queries, we can implement $O_{j}$.
	Applying \cref{lemma:sparse} once more, we get that at most
	\begin{align*}
		\Delta^{3j} \cdot \left( \Delta + \Delta^{\frac{1}{10}} \right) 
		= \Delta^{3j + 1} + \Delta^{3j + \frac{1}{10}} 
		\leq 2\Delta^{3j + 1}\leq \Delta^{3(j + 1)}
	\end{align*}
	queries are needed to simulate phase $j + 1$.
	The claim follows by induction.
\end{proof}

\begin{theorem}
	\label{thm:sqrt}
	There is an LCA algorithm that solves the MIS problem with $\Delta^{\bigO\left( \sqrt{\log \Delta} \right) }$ queries with high probability.
\end{theorem}
\begin{proof}
	By \cref{lemma:learn}, we get that simulating $\bigO(\log \Delta + \log (1 / \eps))$ rounds, i.e., 
	\[
		\bigO \left( \frac{\log \Delta + \log (1 / \eps)}{\sqrt{\log \Delta}} \right)
	\]
	phases, requires\ju{again, maybe a more direct proposition}
	\[
		\Delta^{\bigO \left( \frac{\log \Delta + \log (1 / \eps)}{\sqrt{\log \Delta}} \right)}
	\]
	queries.
	By combining this with \cref{thm:beepruntime} and setting $\eps = 1/n^{c}$, we get an LCA algorithm that outputs an MIS with probability $1 - 1/\Delta^{c}$ with query complexity
	\[
		\Delta^{ \bigO \left( \frac{ \log \Delta + \log \Delta^{c} }{ \sqrt{ \log \Delta } } \right) }  = \Delta^{\bigO \left( \frac{ \log \Delta }{ \sqrt{ \log \Delta } } \right)} = \Delta^{\bigO( \sqrt{\log \Delta} )} \ .
	\]
	Similarly, we get an MIS algorithm with success probability $1 - 1/n^{c}$ and with query complexity
	\[
		\Delta^{\bigO\left( \sqrt{\log \Delta} + \frac{\log n}{\sqrt{\log \Delta}} \right)} 
		= \Delta^{\bigO\left( \sqrt{\log \Delta}\left( 1 + \frac{\log n}{\log \Delta} \right) \right)} \ .
	\]
\end{proof}

==> temp.tex <==

\section{Sparsification}

% What we want:
% \begin{enumerate}
% 	\item nodes that get sampled in some iteration in a phase
% 	\item nodes that get marked in some iteration in a phase
% 	\item low degree
% \end{enumerate}
% Problem:
% A heavy node might get sampled. 
% Solution: heavy nodes are stalling. We can predict what they do.

% \paragraph{Sparsified Graph $\Gt$.}
Every node draws $O(\log^2 \Delta)$ random bits such that there are $c \log \Delta$ bits of fresh randomness for each of the  $O(\log \Delta)$ iterations of the MIS algorithm for desirably large constant $c$.
For iteration $t$, let $r_t(v)$ denote a uniformly chosen random number, with $c \log \Delta$-bit precision, from the interval $[0, 1]$.
Now, we can derive the outcome of the random sampling and random marking by checking whether $p_t(v) < r_t(v)$.\ju{using the same randomness for makring and sampling is ok?}
We denote an interval of iterations from $t$ to $t'$ by $[t, t']$ and refer to this inter to as a phase if it corresponds to a phase in Algorithm~\ref{alg:localmis}.
The sparsified graph $\Gt$ for phase $[t, t']$ is constructed as follows.
If $[t, t']$ is the $i$:th phase, we denote $\Gt$ by $\Gi$.

\paragraph{Nodes in $\Gt$.}
Let $u$ be a node for which $r_i(u) < p_{t}(u) \cdot 2^{\sqrt{\log \Delta} / 10}$ for some $i \in [t, t']$.
Notice that if this condition is not satisfied, node $u$ will not get marked nor sampled in phase $[t, t']$.
We say that a node satisfying this condition is \emph{relevant}.
We say that node $u$ is \emph{light}, if $d_t(u) < 2^{\sqrt{\log \Delta} / 5 + 1}$.
Otherwise, $u$ is \emph{heavy}.
For a light node $u$, we have that $d_{i}(u) < 2^{\sqrt{\log \Delta} / 5 + \sqrt{\log \Delta} / 10 + 1} =  2^{(3/10) \cdot \sqrt{\log \Delta} + 1}$ for all iterations $i \in [t, t']$.
% By Lemma~\ref{lemma:notoff} and a union bound over all iterations, we get for all $i \in [t, t']$ with probability at most $1 - 1/\Delta^{99}$ that
We say that $u$ is \emph{good} if the following inequality holds for all $i \in [t, t']$ and otherwise, it is bad.
\[
	\hat{d}_{i}(u) \leq 2^{(3/10) \cdot \sqrt{\log \Delta} + 2} = 4 \cdot 2^{(3/10) \cdot \sqrt{\log \Delta}} \ .
\]
All relevant light nodes that are good are added to $\Gt$.
For a relevant heavy node $u$, we create $d$ virtual copies, where $d$ is the number of relevant light nodes that are good and connected to $u$ in the original graph.
All these copies are added to $\Gt$.

\paragraph{Edges in $\Gt$.} 
If two light nodes $u$ and $w$ are connected in the original graph, we add the edge $\{ u, w \}$ to $\Gt$.
Each copy of a relevant heavy node $w$ gets an edge to exactly one of the light nodes that $w$ is connected to in the original graph.
Hence, every heavy node in $\Gt$ has degree one and is connected to a light node.

\paragraph{Labels in $\Gt$.}
Every node $u$ in $\Gt$ is labeled with its random bits $r = (r_t, \ldots, r_{t'})$.
In addition, each copy of a relevant heavy node $w$ is labeled as stalling in $\Gt$.
This label can be thought of as a bit string appended to the identifier of the node. 

\begin{observation}
	Given the $p_t(v)$ values for all nodes $v$, the graph $\Gt$ can be constructed in one communication round.
	\label{obs:construct}
\end{observation}

\begin{lemma}
	\label{lemma:MISsparsify}
	Let $x = \sqrt{\log \Delta} / 10$.
	A light node $v$ is bad in phase $[t, t']$ with probability\footnote{notice that to get the probability $1/\Delta^{100}$, we can insert any $x \geq \log \log \Delta$.} at most $e^{-2^{2x}} \ll 1/\Delta^{100}$.
	Furthermore, the event that a node is bad is independent of the randomness of nodes outside of its $2$-hop neighborhood.
\end{lemma} 
\begin{proof}
	By definition, $d_t(v) < 2^{\sqrt{\log \Delta} / 5 + 1} = 2^{2x + 1}$.\ju{check numbers for corner cases}
	Since the $d_t(v)$ value increases by at most a factor of two in every iteration, we get that $d_i(v) < 2^{2x + 1} \cdot 2^{x} = 2^{3x + 1}$ for any iteration $i \in [t, t']$.
	The expected value $\expect[\hat{d}_i(v)] = \mu$ is therefore bounded from above by $2^{3x + 1}$ and thus, by a Chernoff bound, we have
	\[
		\pr(\hat{d}_i(v) > 2\mu) = \pr\left( \hat{d}_i(v) > 2^{3x + 2} \right) < e^{-2^{3x + 1} \cdot (1/3)} = e^{-2^{(3/10)\sqrt{\log \Delta} + 1}} \ .
	\]
	
	Node $v$ is bad if there is at least one iteration $i$ such that $\hat{d}_i(v) > 2^{(3/10) \sqrt{\log \Delta} + 2} = 2^{3x + 2}$.
	By a union bound we get that the probability of node $v$ being bad is at most 
	\[
		O(\log \Delta) \cdot e^{-2^{3x}} < e^{-2^{2x}} \ll 1/\Delta^{100} \ . \qedhere
	\]
	We get the independence by observing that $2^{3x + 1}$ is an upper bound for $\hat{d}_i(v)$ regardless of the random choices of its neighbors.
	Thus, the bad event only depends on the randomness of the neighbors of $v$ in the corresponding iteration.
\end{proof}

\begin{observation}
	\label{lemma:degsize}
	The maximum degree of $\Gt$ is $O\left( 2^{(4/10) \sqrt{\log \Delta}} \right)$.
	Furthermore, the number of nodes in the $(\sqrt{\log \Delta}/10)$-hop neighborhood of any node node $v$ is bounded from above by $\sqrt{\Delta}$.
\end{observation}
\begin{proof}
	By definition, all (copies of) heavy nodes in $\Gt$ have degree exactly $1$.
	Since we only picked good light nodes $u$, we have that $\hat{d}_{i}(u) \leq 4\cdot 2^{(3/10) \cdot \sqrt{\log \Delta}}$ for all $i \in [t, t']$.
	Thus, the number of sampled and marked neighbors of $u$ is bounded from above by $800 \log \Delta \cdot \hat{d}_{i}(u)$ for any iteration $i$.
	Summing up over all iterations, for a sufficiently large $\Delta$, we can bound the number of neighbors of $u$ by
	\[
		O(\sqrt{ \log \Delta}) \cdot 800 \log \Delta \cdot \hat{d}_{i}(u) = O\left( 2^{(4/10) \sqrt{\log \Delta}} \right) \ . \qedhere
	\]
	For the second claim, the number of neighbors in the $(\sqrt{\log \Delta}/10)$-hop neighborhood of any node $v$ is at mots 
	\[
		\left( 2^{(4/10) \sqrt{\log \Delta}} \right)^{\sqrt{\log \Delta}/10} = \left(2^{(4/100) \log \Delta} \right) \ll \sqrt{\Delta} \ . 
	\]
\end{proof}


\begin{lemma}
	Consider a phase $[t, t']$. 
	If node $v$ learns its $(t' - t)$-hop neighborhood in $\Gt$, it can simulate its behavior in iterations in $[t, t']$.
	In particular, node $v$ learns $p_{t'}(v)$ and whether it joined the MIS.
	\label{lemma:localcorrectness}
\end{lemma}
\begin{proof}
	We argue by induction on the iteration index that the behavior of $v$ can be derived solely based on the nodes in $\Gt$.	
	For the base case, i.e., iteration $t$, consider a non-stalling node $v$ and a neighbor $u$ of $v$.
	According to the construction of $\Gt$, if $u$ is sampled or marked in iteration $t$, it belongs to $\Gt$.	
	Node $v$ can learn the $p_t(u)$ value, the random bits used in iteration $t$, whether $u$ is stalling by looking at the label of $u$.
	With this information, $v$ can deduce whether $u$ is marked in iteration $t$.
	If any neighbor of $v$ is marked, then $v$ cannot join the MIS.
	Conversely, if no neighbor is marked and $v$ is, then $v$ joins the MIS.	
	Furthermore, since $\Gt$ contains all the marked neighbors of $v$ in iteration $t$, node $v$ can derive $\hat{d}_t(v)$ from the labels of its neighbors.
	Thus, node $v$ can determine $p_{t + 1}(v)$.
	The argumentation is the same for a stalling node $v$, except that a stalling node must consider the neighbors of all of its copies and it does not join the MIS even if it is marked and none of its neighbors are.
	
	Assume then that the claim holds for iteration $t \leq i < t'$.
	Due to the construction of $\Gt$ $v$ can learn the random bits, and whether the neighbor is stalling in iteration $i$ by looking at the labels of its neighbors.
	By the induction hypothesis, $v$ knows the $p_{i}(u)$ values of all of its neighbors and whether they joined the MIS or not.
	In case $v$ or a neighbor joined the MIS, we are done.
	The remainder of the claim follows from analogous considerations as in the base case.
\end{proof}



\subsection{Simulation in the low memory MPC Model}
For the simulation in the low memory MPC model, we split the execution of Algorithm~\ref{} into $\log \log \Delta + 1$ steps, where in step $i$, we only consider nodes with degree at least $\Delta^{2^{-i}}$.
Let $\Delta_i$ be the maximum degree and $n_i$ the number of nodes in the graph that remains in step $i$.\ju{$\Delta$ vs $n^{\alpha}$?}


\begin{lemma}
	Every node $v$ can learn its $(\sqrt{\log \Delta_i}/10)$-hop neighborhood in the low memory MPC model in $O(\log \log \Delta_i)$ communication rounds.
	In particular, the $(\sqrt{\log \Delta_i}/10)$-hop neighborhood of every node in step $i$ fits into the total memory.
	\label{lemma:learnnbh}
\end{lemma}
\begin{proof}
	Due to the design of the algorithm, we have that the minimum degree of a node $v$ considered in step $i$ is at least $\sqrt{\Delta_i}$ and hence, the total memory we have is at least $n_i \cdot \sqrt{\Delta_i}$.
	By Lemma~\ref{lemma:degsize}, this implies that the $(\sqrt{\log \Delta_i}/10)$-hop neighborhood of any node in this step fits into memory.
	Put otherwise, the total memory suffices to store a copy of the $(\sqrt{\log \Delta_i}/10)$-hop neighborhood of every node in this step.

	Consider the following graph exponentiation procedure~\cite{}.
	In every communication round, each node $u$ informs its neighbors of the nodes contained in $N(u)$.
	Then, every node can add the new nodes it learned about in its neighborhood by adding a virtual edge.
	This way, in $i$ round, node $v$ will be informed about all nodes and edges in its $2^i$-hop neighborhood.
\end{proof}


\begin{theorem}
	Simulation in the low memory MPC model requires $O(\sqrt{\log \Delta} \log \log \Delta + \sqrt{\log \log n})$ communication rounds.
\end{theorem}
\begin{proof}
Let $[t, t']$ be a phase of Algorithm~\ref{}.
Given that we know the $p_t(v)$ value of every node, we can construct graph $\Gt$ in a single communication round.
Combining this observation with lemmas~\ref{lemma:localcorrectness,lemma:MISsparsify,lemma:learnnbh}, we can use Lemma~\ref{} to obtain shattering.
Since the size of the remaining components is ?? and the number of remaining nodes is ??, we can apply the graph exponentiation procedure once more and simulate the deterministic algorithm for MIS designed for these small components by Ghaffari~\ref{}.
This simulation requires every node to know the $2^{O(\sqrt{\log \log n})}$-hop neighborhood resulting in a runtime of $O(\sqrt{\log \log n})$ for the deterministic part.

Putting the randomized and the deterministic part together and summing up over all steps results in a runtime of
\[
	\sum_{i = 1}^{\log \log \Delta + 1} \sqrt{\log \Delta_i} \cdot \log \log \Delta_i = \sum_{i = 1}^{\log \log \Delta + 1} \sqrt{2^{-i} \log \Delta} \cdot \log \log 2^{-i} \Delta = O(\sqrt{\log \Delta} \cdot \log \log \Delta) \ .
\]


\end{proof}


\subsection{Simulation in the LCA Model}
The idea for creating an LCA from the MIS algorithm in the LOCAL model follows in the footsteps of the MPC algorithm.
Lemma~\ref{lemma:MISsparsify} gives us the means to sparsify the graph during the simulation of a phase.
Thus, an LCA for node $v$ can simulate the first $\sqrt{\log \Delta}/10$ iterations by querying the nodes in the $\sqrt{\log \Delta}/10$-hop neighborhood of $v$ that are contained in $\Gt$.

To create an LCA that simulates the second phase, we think of the LCA for the first phase as an oracle that provides a query access to the $p_t(u)$ values of nodes in the original graph $G$.
Through this oracle, we can also figure out whether $u$ belongs to $\Gt$.
More generally, we want to create an oracle $\orci(v)$ that answer the following question:
What is the state of node $v$ in the beginning of phase $i = [t, t']$?
In particular, whether $v$ joined the MIS and what is $p_t(v)$.\ju{stalling?}

\paragraph{Oracle $\orci(v))$.}
Since $p_0(u)$ is $1/2$ for all nodes $u$, oracle $\orc_0(v)$ can be implemented without any queries given that $v$ knows its neighbors.
For $i > 0$, oracle $\orci(v)$ is implemented recursively as follows.
For each neighbor $u$ of $v$, query the state of $u$ with $\orc_{i - 1}(u)$.
From the $1$-hop neighborhood, node $v$ can decide whether it is stalling or not.
Furthermore, can deduce which neighbors belong to $G_{i - 1}$.
All such neighbors are queried with $\orc_{i - 1}$ until the $(\sqrt{\log \Delta}/10)$-hop neighborhood of $v$ in $G_{i - 1}$ is discovered.

Let us denote the query complexity of simulating phase $i$ by $Q(i)$ and the query complexity of oracle $\orci(u)$ by $Q(\orci)$.
\begin{lemma}
	The oracle $\orci(v)$ for phase $i$ for node $v$ requires at most $Q(i - 1) \cdot \Delta^{3/2}$ queries.
	\label{lemma:onephasequeries}
\end{lemma}
\begin{proof}
	According to the design of $\orci(v)$, we query every neighbor of every node in the $(\sqrt{\log \Delta}/10)$-hop neighborhood of $v$ in $G_{i - 1}$.
	Notice that we do not query any nodes that $(\sqrt{\log \Delta}/10)$-hop neighborhood of $v$ in $G_{i - 1}$ and that are not adjacent to any node in this neighborhood.
	Now, from Lemma~\ref{lemma:degsize}, we get that the number of nodes that are queried in total is at most $\sqrt{\Delta} \cdot \Delta = \Delta^{3/2}$.
\end{proof}

\begin{theorem}
	There is an LCA for the maximal independent set problem with query complexity $\Delta^{O(\sqrt{\log \Delta})} \cdot \log n$ queries.
\end{theorem}
\begin{proof}
	let $T$ denote the runtime of Algorithm~\ref{}.
	Let $x$ be the number of phases and notice that $x = O(\sqrt{\log \Delta})$.
	Using Lemma~\ref{lemma:onephasequeries} can bound the total query complexity of our simulation from above by
	\begin{align*}
		Q(x) & = \Delta^{3/2} \cdot Q(x - 1) = \Delta^{3/2} \cdot \Delta^{3/2} \cdot Q(x - 2) \\
			 & = \prod_{i = 1}^{x} \Delta^{3/2} = \Delta^{O(\sqrt{\log \Delta})} \ .
	\end{align*}
	
	After running these phases, by Lemma~\ref{}, the remaining components are of size at most $O(\Delta^4 \cdot \log n)$.\ju{check polylog}
	Thus, if we can complete our LCA for node $v$ by learning all node in the corresponding component resulting in a total query complexity of $Q(x) \cdot \Delta^{O(1)} \cdot \log n = \Delta^{O(\sqrt{\log \Delta})} \cdot \log n$.
\end{proof}

\section{An Improved LCA for MIS}

\begin{algorithm}
	\caption{Recursive MIS algorithm for node $v$:}
	\label{alg:subphase}
	\begin{algorithmic}
		\Require tor
		\For{iteration $t = 1, 2, \ldots$ until node $v$ is not removed.} 
			\State {\bf Round 1:} Send $p_{t - 1}$ to all neighbors.% \Comment{Round $1$}
			\State Set 
				\[
					p_{t}(v) = 	\begin{cases}
										p_t(v)/2, \hfill \text{if } d_{t - 1}(v) \geq 2 \text{ or if $v$ is stalling} \\
										\min\{ 2p_{t}, 1/2 \}, \hfill \text{otherwise.}
								\end{cases}
				\]
			\If{$d_{t_1} \geq 200 \log \Delta$} 
				\State Let $x$ be the largest positive integer such that $p_{t}(v) \cdot 2^{-x} \geq 100 \log \Delta$.
				\State Stall for $x$ iterations.
			\EndIf
			\State {\bf Round 2:} If $v$ is not stalling, it \emph{marks} itself w.p. $p_{t}(v)$. 
			\State If $v$ is the only marked node in $N(v)$, then $v$ joins the MIS. 
			\State For the rest of the execution, $v$ is removed from the graph along with its neighbors.
		\EndFor
	\end{algorithmic}
\end{algorithm} 

